MURPHY -- A scalable multiresolution framework for scientific computing on 3D block-structured collocated grids

We present the derivation, implementation, and analysis of a multiresolution adaptive grid framework for numerical simulations on octree-based 3D block-structured collocated grids with distributed computational architectures. Our approach provides a consistent handling of non-lifted and lifted interpolating wavelets of arbitrary order demonstrated using second, fourth, and sixth order wavelets, combined with standard finite-difference based discretization operators. We first validate that the wavelet family used provides strict and explicit error control when coarsening the grid, and show that lifting wavelets increase the grid compression rate while conserving discrete moments across levels. Further, we demonstrate that high-order PDE discretization schemes combined with sufficiently high order wavelets retain the expected convergence order even at resolution jumps. We then simulate the advection of a scalar to analyze convergence for the temporal evolution of a PDE. The results shows that our wavelet-based refinement criterion is successful at controlling the overall error while the coarsening criterion is effective at retaining the relevant information on a compressed grid. Our software exploits a block-structured grid data structure for efficient multi-level operations, combined with a parallelization strategy that relies on a one-sided MPI-RMA communication approach with active PSCW synchronization. Using performance tests up to 16,384 cores, we demonstrate that this leads to a highly scalable performance. The associated code is available under a BSD-3 license at https://github.com/vanreeslab/murphy.

==> wavelet_0_main_aux.tex <==



==> wavelet_0_supp_aux.tex <==



==> wavelet_s4_multilevel_moments.tex <==
\section{Moment conservation on multiresolution grids.}

Lifted wavelet schemes are designed to conserve the moment of a function which lies in the multiresolution analysis during refinement or coarsening. Consequently it is important to be able to calculate this moment for a function represented on a multiresolution grid. 

Any function $f \in V^j$ can be expanded as a sum of the basis functions $\{\varphi^j_k\}$, so that 
\begin{equation}
    f = \sum_k \lambda_k^j \varphi_k^j.
\end{equation}
With this representation, any moment of $f$ can be expressed as a linear combination of the scaling coefficients $\{\lambda_k^j\}$. The weights in this linear combination are determined by integrating over the above, so that
\begin{equation}
    \int x^p f\, dx = \sum_k \lambda_k^j \int x^p \varphi_k^j \,dx. 
\end{equation}
For interpolating scaling functions of order $N$ on a regular grid, the moments of the mother scaling function $\int x^p \varphi \,dx$ vanish for $0 < p < N$ \citep{Sweldens:1996}, so that the above simplifies to
\begin{equation}
    \int x^p f\, dx = \sum_k \lambda_k^j (x_k^j)^p \quad \text{for } 0 < p < N.
\end{equation}
On a uniform grid with resolution level $j$, all of the scaling coefficients $\{\lambda_j^k\}$ are readily available on the grid, and the above is a convenient strategy for calculating the moment of a function represented on the grid.

For a multiresolution grid with finest level $j$, any function represented on the grid is assumed to be a member of $V^j$. However, an expansion of $f$ in the basis $\{\varphi^j_k\}$ is not readily available, because not all level $j$ scaling coefficients are present on the grid.  This can be remedied by refining the entire grid to level $j$, which produces a more convenient representation of $f$ without altering the function itself. However, full refinement is expensive, and can be avoided using the strategy outlined below.

Consider for simplicity a two-level grid with levels $j$ and $j+1$, on which we wish to calculate the integral of a function $f$. Let $L^{j+1}$ be the set of points represented on the finer resolution level (including resolution boundaries), and let $K$ be the set of points which coincide with a level $j$ scaling coefficient (even indices). The level $j+1$ expansion of the integral of $f$ can be written
\begin{equation}
    \int f \,dx = \sum_{l \in L^{j+1}} \lambda_l^{j+1} dV^{j+1} + \sum_{l \notin L^{j+1}} \lambda_l^{j+1} dV^{j+1},
\end{equation}
where $dV^j = \int \phi_k^j \,dx$ is the standard volume element on level $j$. The scaling coefficients in the first sum are available directly from the grid, while the scaling coefficients in the second sum are not. Because all level $j$ wavelet coefficients $\gamma_m^j$ near and inside the coarse region are assumed to be zero, the scaling coefficients $\lambda_l^{j+1}$ which coincide with a coarse point $x_k^j$ are equal to the corresponding level $j$ scaling coefficient $\lambda_k^j$. Consequently, all fine scaling coefficients which lie in $K$, $\{\lambda_k^{j+1}: k \in K\}$, are available on the grid. This fact is used during refinement of the grid, in which the missing scaling coefficients on level $j+1$ can be calculated from information on the grid using the order $N$ refinement relation
$ \lambda_l^{j+1} = \sum_{k \in K} h_{k,l} \lambda_k^{j+1}. $
Substituting this refinement relation into the second summation from our earlier expansion gives
\begin{equation}
\begin{aligned}
    \sum_{l \notin L^{j+1}} \lambda_l^{j+1} dV^{j+1} &= \sum_{l \notin L^{j+1}} \sum_{k \in K} h_{k,l} \lambda_k^{j+1} dV^{j+1} \\
    &= \sum_{k \in K}  \big(\sum_{l \notin L^{j+1}} h_{k,l} dV^{j+1}\big) \lambda_k^{j+1}.
\end{aligned}
\end{equation}
All of the $\{\lambda_k^{j+1}\}$ are values contained on the multiresolution grid, and the weight in parentheses represents a modified quadrature weight which must be applied to all points in $K$. Noting that $h_{k,l}$ has compact support for fixed $k$, this weighting simplifies considerably for points $k \in K$ that are not near the resolution boundary.
\begin{itemize}
    \item For points $k$ on the fine level for which $\mathrm{Supp}(h_{k,l}) \subset L^{j+1}$, the weighting reduces to zero.
    \item For points $k$ on the coarse level for which $\mathrm{Supp}(h_{k,l}) \subset (L^{j+1})^c$, the weighting reduces to $\sum_l h_{k,l} dV^{j+1}$, which can be further simplified to $2^d dV^{j+1} = dV^j$.
\end{itemize} 
Thus most points on the fine level do not participate in this sum, and most points on the coarse level are weighted by their local volume element $dV^j$. All modifications to the standard quadrature one each level occur in a narrow regions surrounding the resolution boundary.

For moments beyond the zeroth, the weighting scheme is modified by an additional position term:
\begin{equation}
    \int x^p f \,dx = \sum_{l \in L^{j+1}} \lambda_l^{j+1} (x_l^{j+1})^p dV^{j+1} + \sum_{k \in K}  \big[\sum_{l \notin L^{j+1}} h_{k,l} (x_l^{j+1})^p dV^{j+1}\big] \lambda_k^{j+1}.
\end{equation}
On grids with more than two levels, the ``balanced grid" criteria ensures that no more than two resolutions meet at any resolution boundary. The procedure above can be generalized to grids with three or more levels by applying the necessary corrections locally near each resolution boundary, adapting the levels $j$ and $j+1$ to match the local coarser and finer levels.













